Adaptive Testing for Specification Coverage

Ensuring correctness of cyber-physical systems (CPS) is an extremely challenging task that is in practice often addressed with simulation based testing. Formal specification languages, such as Signal Temporal Logic (STL), are used to mathematically express CPS requirements and thus render the simulation activity more systematic and principled. We propose a novel method for adaptive generation of tests with specification coverage for STL. To achieve this goal, we devise cooperative reachability games that we combine with numerical optimization to create tests that explore the system in a way that exercise various parts of the specification. To the best of our knowledge our approach is the first adaptive testing approach that can be applied directly to MATLAB\texttrademark\; Simulink/Stateflow models. We implemented our approach in a prototype tool and evaluated it on several illustrating examples and a case study from the avionics domain, demonstrating the effectiveness of adaptive testing to (1) incrementally build a test case that reaches a test objective, (2) generate a test suite that increases the specification coverage, and (3) infer what part of the specification is actually implemented.

==> abstract.tex <==
\begin{abstract}
Ensuring correctness of cyber-physical systems (CPS) is an extremely challenging task that is in practice often 
addressed with simulation-based testing. Formal specification languages, such as Signal Temporal Logic (STL), 
are used to mathematically express CPS requirements and thus render the simulation activity more 
systematic and principled. We propose a novel method for adaptive generation of 
tests with specification coverage for STL. To achieve this goal, we devise cooperative reachability games 
that we combine with numerical optimization to create tests that explore the system 
in a way that exercise various parts of the specification. To the best of our knowledge our approach is the first 
adaptive testing approach that can be applied directly to MATLAB\texttrademark\; Simulink/Stafeflow models. 
%
We implemented our approach in a prototype tool and evaluated it on several illustrating examples and 
a case study from the avionics domain, demonstrating the effectiveness of adaptive testing to (1) 
incrementally build a test case that reaches a test objective, (2) generate a test suite that increases 
the specification coverage, and (3) infer what part of the specification is actually implemented. 
\end{abstract}

==> coverage.tex <==
\section{Specification Coverage}
\label{sec:coverage}

A {\em test coverage criterion} $C$ defines a set of testing requirements that a {\em test suite} $T$ must fulfil. Given a 
test $t \in T$ and a requirement $c \in C$, we denote by $t \models c$ the fact that $t$ {\em satisfies} the criterion $c$. 
We define by $R(T,C) = \{ c~|~t\in T, c \in C \text{ and } t \models c \}$ the set of test coverage requirements from the 
criterion $C$ satisfied by the test suite $T$. The {\em test coverage} of $T$, denoted by $K(C,T)$ is the ratio between 
the number of testing requirements in $C$ that $T$ fulfills and the total number of testing requirements defined by $C$, 
that is $K(C,T) = \frac{|R(T,C)|}{|C|}$.
